Lattice Chiral Schwinger Model: Selected Results

We discuss a method for regularizing chiral gauge theories. The idea is to formulate the gauge fields on the lattice, while the fermion determinant is regularized and computed in the continuum. A simple effective action emerges which lends itself to numerical simulations.

==> fig1.tex <==
% GNUPLOT: LaTeX picture with Postscript
\setlength{\unitlength}{0.1bp}
\special{!
%!PS-Adobe-2.0 EPSF-2.0
%%Title: 'imdet_cont_buck.tex'
%%Creator: gnuplot
%%DocumentFonts: 
%%BoundingBox: 0 0 360 216
%%Orientation: Landscape
%%EndComments
/gnudict 120 dict def
gnudict begin
/Color false def
/Solid false def
/gnulinewidth 5.000 def
/vshift -33 def
/dl {10 mul} def
/hpt 31.5 def
/vpt 31.5 def
/M {moveto} bind def
/L {lineto} bind def
/R {rmoveto} bind def
/V {rlineto} bind def
/vpt2 vpt 2 mul def
/hpt2 hpt 2 mul def
/Lshow { currentpoint stroke M
  0 vshift R show } def
/Rshow { currentpoint stroke M
  dup stringwidth pop neg vshift R show } def
/Cshow { currentpoint stroke M
  dup stringwidth pop -2 div vshift R show } def
/DL { Color {setrgbcolor Solid {pop []} if 0 setdash }
 {pop pop pop Solid {pop []} if 0 setdash} ifelse } def
/BL { stroke gnulinewidth 2 mul setlinewidth } def
/AL { stroke gnulinewidth 2 div setlinewidth } def
/PL { stroke gnulinewidth setlinewidth } def
/LTb { BL [] 0 0 0 DL } def
/LTa { AL [1 dl 2 dl] 0 setdash 0 0 0 setrgbcolor } def
/LT0 { PL [] 0 1 0 DL } def
/LT1 { PL [4 dl 2 dl] 0 0 1 DL } def
/LT2 { PL [2 dl 3 dl] 1 0 0 DL } def
/LT3 { PL [1 dl 1.5 dl] 1 0 1 DL } def
/LT4 { PL [5 dl 2 dl 1 dl 2 dl] 0 1 1 DL } def
/LT5 { PL [4 dl 3 dl 1 dl 3 dl] 1 1 0 DL } def
/LT6 { PL [2 dl 2 dl 2 dl 4 dl] 0 0 0 DL } def
/LT7 { PL [2 dl 2 dl 2 dl 2 dl 2 dl 4 dl] 1 0.3 0 DL } def
/LT8 { PL [2 dl 2 dl 2 dl 2 dl 2 dl 2 dl 2 dl 4 dl] 0.5 0.5 0.5 DL } def
/Pnt { stroke [] 0 setdash
   gsave 1 setlinecap M 0 0 V stroke grestore } def
/Dia { stroke [] 0 setdash 2 copy vpt add M
  hpt neg vpt neg V hpt vpt neg V
  hpt vpt V hpt neg vpt V closepath stroke
  Pnt } def
/Pls { stroke [] 0 setdash vpt sub M 0 vpt2 V
  currentpoint stroke M
  hpt neg vpt neg R hpt2 0 V stroke
  } def
/Box { stroke [] 0 setdash 2 copy exch hpt sub exch vpt add M
  0 vpt2 neg V hpt2 0 V 0 vpt2 V
  hpt2 neg 0 V closepath stroke
  Pnt } def
/Crs { stroke [] 0 setdash exch hpt sub exch vpt add M
  hpt2 vpt2 neg V currentpoint stroke M
  hpt2 neg 0 R hpt2 vpt2 V stroke } def
/TriU { stroke [] 0 setdash 2 copy vpt 1.12 mul add M
  hpt neg vpt -1.62 mul V
  hpt 2 mul 0 V
  hpt neg vpt 1.62 mul V closepath stroke
  Pnt  } def
/Star { 2 copy Pls Crs } def
/BoxF { stroke [] 0 setdash exch hpt sub exch vpt add M
  0 vpt2 neg V  hpt2 0 V  0 vpt2 V
  hpt2 neg 0 V  closepath fill } def
/TriUF { stroke [] 0 setdash vpt 1.12 mul add M
  hpt neg vpt -1.62 mul V
  hpt 2 mul 0 V
  hpt neg vpt 1.62 mul V closepath fill } def
/TriD { stroke [] 0 setdash 2 copy vpt 1.12 mul sub M
  hpt neg vpt 1.62 mul V
  hpt 2 mul 0 V
  hpt neg vpt -1.62 mul V closepath stroke
  Pnt  } def
/TriDF { stroke [] 0 setdash vpt 1.12 mul sub M
  hpt neg vpt 1.62 mul V
  hpt 2 mul 0 V
  hpt neg vpt -1.62 mul V closepath fill} def
/DiaF { stroke [] 0 setdash vpt add M
  hpt neg vpt neg V hpt vpt neg V
  hpt vpt V hpt neg vpt V closepath fill } def
/Pent { stroke [] 0 setdash 2 copy gsave
  translate 0 hpt M 4 {72 rotate 0 hpt L} repeat
  closepath stroke grestore Pnt } def
/PentF { stroke [] 0 setdash gsave
  translate 0 hpt M 4 {72 rotate 0 hpt L} repeat
  closepath fill grestore } def
/Circle { stroke [] 0 setdash 2 copy
  hpt 0 360 arc stroke Pnt } def
/CircleF { stroke [] 0 setdash hpt 0 360 arc fill } def
/C0 { BL [] 0 setdash 2 copy moveto vpt 90 450  arc } bind def
/C1 { BL [] 0 setdash 2 copy        moveto
       2 copy  vpt 0 90 arc closepath fill
               vpt 0 360 arc closepath } bind def
/C2 { BL [] 0 setdash 2 copy moveto
       2 copy  vpt 90 180 arc closepath fill
               vpt 0 360 arc closepath } bind def
/C3 { BL [] 0 setdash 2 copy moveto
       2 copy  vpt 0 180 arc closepath fill
               vpt 0 360 arc closepath } bind def
/C4 { BL [] 0 setdash 2 copy moveto
       2 copy  vpt 180 270 arc closepath fill
               vpt 0 360 arc closepath } bind def
/C5 { BL [] 0 setdash 2 copy moveto
       2 copy  vpt 0 90 arc
       2 copy moveto
       2 copy  vpt 180 270 arc closepath fill
               vpt 0 360 arc } bind def
/C6 { BL [] 0 setdash 2 copy moveto
      2 copy  vpt 90 270 arc closepath fill
              vpt 0 360 arc closepath } bind def
/C7 { BL [] 0 setdash 2 copy moveto
      2 copy  vpt 0 270 arc closepath fill
              vpt 0 360 arc closepath } bind def
/C8 { BL [] 0 setdash 2 copy moveto
      2 copy vpt 270 360 arc closepath fill
              vpt 0 360 arc closepath } bind def
/C9 { BL [] 0 setdash 2 copy moveto
      2 copy  vpt 270 450 arc closepath fill
              vpt 0 360 arc closepath } bind def
/C10 { BL [] 0 setdash 2 copy 2 copy moveto vpt 270 360 arc closepath fill
       2 copy moveto
       2 copy vpt 90 180 arc closepath fill
               vpt 0 360 arc closepath } bind def
/C11 { BL [] 0 setdash 2 copy moveto
       2 copy  vpt 0 180 arc closepath fill
       2 copy moveto
       2 copy  vpt 270 360 arc closepath fill
               vpt 0 360 arc closepath } bind def
/C12 { BL [] 0 setdash 2 copy moveto
       2 copy  vpt 180 360 arc closepath fill
               vpt 0 360 arc closepath } bind def
/C13 { BL [] 0 setdash  2 copy moveto
       2 copy  vpt 0 90 arc closepath fill
       2 copy moveto
       2 copy  vpt 180 360 arc closepath fill
               vpt 0 360 arc closepath } bind def
/C14 { BL [] 0 setdash 2 copy moveto
       2 copy  vpt 90 360 arc closepath fill
               vpt 0 360 arc } bind def
/C15 { BL [] 0 setdash 2 copy vpt 0 360 arc closepath fill
               vpt 0 360 arc closepath } bind def
/Rec   { newpath 4 2 roll moveto 1 index 0 rlineto 0 exch rlineto
       neg 0 rlineto closepath } bind def
/Square { dup Rec } bind def
/Bsquare { vpt sub exch vpt sub exch vpt2 Square } bind def
/S0 { BL [] 0 setdash 2 copy moveto 0 vpt rlineto BL Bsquare } bind def
/S1 { BL [] 0 setdash 2 copy vpt Square fill Bsquare } bind def
/S2 { BL [] 0 setdash 2 copy exch vpt sub exch vpt Square fill Bsquare } bind def
/S3 { BL [] 0 setdash 2 copy exch vpt sub exch vpt2 vpt Rec fill Bsquare } bind def
/S4 { BL [] 0 setdash 2 copy exch vpt sub exch vpt sub vpt Square fill Bsquare } bind def
/S5 { BL [] 0 setdash 2 copy 2 copy vpt Square fill
       exch vpt sub exch vpt sub vpt Square fill Bsquare } bind def
/S6 { BL [] 0 setdash 2 copy exch vpt sub exch vpt sub vpt vpt2 Rec fill Bsquare } bind def
/S7 { BL [] 0 setdash 2 copy exch vpt sub exch vpt sub vpt vpt2 Rec fill
       2 copy vpt Square fill
       Bsquare } bind def
/S8 { BL [] 0 setdash 2 copy vpt sub vpt Square fill Bsquare } bind def
/S9 { BL [] 0 setdash 2 copy vpt sub vpt vpt2 Rec fill Bsquare } bind def
/S10 { BL [] 0 setdash 2 copy vpt sub vpt Square fill 2 copy exch vpt sub exch vpt Square fill
       Bsquare } bind def
/S11 { BL [] 0 setdash 2 copy vpt sub vpt Square fill 2 copy exch vpt sub exch vpt2 vpt Rec fill
       Bsquare } bind def
/S12 { BL [] 0 setdash 2 copy exch vpt sub exch vpt sub vpt2 vpt Rec fill Bsquare } bind def
/S13 { BL [] 0 setdash 2 copy exch vpt sub exch vpt sub vpt2 vpt Rec fill
       2 copy vpt Square fill Bsquare } bind def
/S14 { BL [] 0 setdash 2 copy exch vpt sub exch vpt sub vpt2 vpt Rec fill
       2 copy exch vpt sub exch vpt Square fill Bsquare } bind def
/S15 { BL [] 0 setdash 2 copy Bsquare fill Bsquare } bind def
/D0 { gsave translate 45 rotate 0 0 Box stroke grestore } bind def
/D1 { gsave translate 45 rotate 0 0 S1 stroke grestore } bind def
/D2 { gsave translate 45 rotate 0 0 S2 stroke grestore } bind def
/D3 { gsave translate 45 rotate 0 0 S3 stroke grestore } bind def
/D4 { gsave translate 45 rotate 0 0 S4 stroke grestore } bind def
/D5 { gsave translate 45 rotate 0 0 S5 stroke grestore } bind def
/D6 { gsave translate 45 rotate 0 0 S6 stroke grestore } bind def
/D7 { gsave translate 45 rotate 0 0 S7 stroke grestore } bind def
/D8 { gsave translate 45 rotate 0 0 S8 stroke grestore } bind def
/D9 { gsave translate 45 rotate 0 0 S9 stroke grestore } bind def
/D10 { gsave translate 45 rotate 0 0 S10 stroke grestore } bind def
/D11 { gsave translate 45 rotate 0 0 S11 stroke grestore } bind def
/D12 { gsave translate 45 rotate 0 0 S12 stroke grestore } bind def
/D13 { gsave translate 45 rotate 0 0 S13 stroke grestore } bind def
/D14 { gsave translate 45 rotate 0 0 S14 stroke grestore } bind def
/D15 { gsave translate 45 rotate 0 0 S15 stroke grestore } bind def
/BoxFill { gsave Rec 1 setgray fill grestore } def
end
%%EndProlog
}
\begin{picture}(3600,2160)(0,0)
\special{"
gnudict begin
gsave
0 0 translate
0.100 0.100 scale
0 setgray
newpath
LTb
613 447 M
63 0 V
2761 0 R
-63 0 V
613 740 M
63 0 V
2761 0 R
-63 0 V
613 1033 M
63 0 V
2761 0 R
-63 0 V
613 1327 M
63 0 V
2761 0 R
-63 0 V
613 1620 M
63 0 V
2761 0 R
-63 0 V
613 1913 M
63 0 V
2761 0 R
-63 0 V
613 300 M
0 63 V
0 1697 R
0 -63 V
1016 300 M
0 63 V
0 1697 R
0 -63 V
1420 300 M
0 63 V
0 1697 R
0 -63 V
1823 300 M
0 63 V
0 1697 R
0 -63 V
2227 300 M
0 63 V
0 1697 R
0 -63 V
2630 300 M
0 63 V
0 1697 R
0 -63 V
3034 300 M
0 63 V
0 1697 R
0 -63 V
3437 300 M
0 63 V
0 1697 R
0 -63 V
613 300 M
2824 0 V
0 1760 V
-2824 0 V
613 300 L
LT5
2594 1947 Circle
3303 729 Circle
2630 667 Circle
2227 638 Circle
1958 622 Circle
1766 612 Circle
1622 605 Circle
1510 601 Circle
1420 597 Circle
LT1
613 582 M
27 0 V
27 0 V
28 0 V
27 0 V
27 0 V
27 1 V
27 0 V
27 0 V
28 0 V
27 1 V
27 0 V
27 1 V
27 0 V
27 1 V
28 0 V
27 1 V
27 0 V
27 1 V
27 1 V
27 0 V
28 1 V
27 1 V
27 0 V
27 1 V
27 1 V
27 1 V
28 1 V
27 1 V
27 1 V
27 1 V
27 1 V
27 1 V
28 1 V
27 1 V
27 1 V
27 1 V
27 1 V
27 1 V
28 2 V
27 1 V
27 1 V
27 2 V
27 1 V
27 1 V
28 2 V
27 1 V
27 1 V
27 2 V
27 1 V
27 2 V
28 1 V
27 2 V
27 2 V
27 1 V
27 2 V
27 1 V
28 2 V
27 2 V
27 2 V
27 1 V
27 2 V
27 2 V
28 2 V
27 2 V
27 2 V
27 1 V
27 2 V
27 2 V
28 2 V
27 2 V
27 2 V
27 3 V
27 2 V
27 2 V
28 2 V
27 2 V
27 2 V
27 3 V
27 2 V
27 2 V
28 2 V
27 3 V
27 2 V
27 3 V
27 2 V
27 2 V
28 3 V
27 3 V
27 2 V
27 3 V
27 2 V
27 3 V
28 3 V
27 2 V
27 3 V
27 3 V
27 3 V
27 3 V
28 2 V
LT6
2594 1847 CircleF
1958 1514 CircleF
3303 1609 CircleF
2630 1549 CircleF
2227 1525 CircleF
1766 1507 CircleF
1622 1502 CircleF
1510 1499 CircleF
1420 1497 CircleF
LT3
613 1488 M
27 0 V
27 0 V
28 0 V
27 0 V
27 0 V
27 0 V
27 0 V
27 0 V
28 1 V
27 0 V
27 0 V
27 0 V
27 1 V
27 0 V
28 0 V
27 0 V
27 1 V
27 0 V
27 1 V
27 0 V
28 0 V
27 1 V
27 0 V
27 1 V
27 0 V
27 1 V
28 0 V
27 1 V
27 1 V
27 0 V
27 1 V
27 0 V
28 1 V
27 1 V
27 1 V
27 0 V
27 1 V
27 1 V
28 1 V
27 0 V
27 1 V
27 1 V
27 1 V
27 1 V
28 1 V
27 1 V
27 1 V
27 1 V
27 1 V
27 1 V
28 1 V
27 1 V
27 1 V
27 2 V
27 1 V
27 1 V
28 1 V
27 2 V
27 1 V
27 1 V
27 2 V
27 1 V
28 1 V
27 2 V
27 1 V
27 2 V
27 1 V
27 2 V
28 2 V
27 1 V
27 2 V
27 2 V
27 2 V
27 1 V
28 2 V
27 2 V
27 2 V
27 2 V
27 2 V
27 2 V
28 2 V
27 2 V
27 3 V
27 2 V
27 2 V
27 3 V
28 2 V
27 2 V
27 3 V
27 2 V
27 3 V
27 3 V
28 2 V
27 3 V
27 3 V
27 3 V
27 3 V
27 3 V
28 3 V
stroke
grestore
end
showpage
}
\put(713,1847){\makebox(0,0)[l]{$t_1=0.00393,~t_2=0.49998 $       }}
\put(713,1947){\makebox(0,0)[l]{$t_{1,2}=0$}}
\put(2025,50){\makebox(0,0){$r=a_f/a$}}
\put(100,1180){%
\special{ps: gsave currentpoint currentpoint translate
270 rotate neg exch neg exch translate}%
\makebox(0,0)[b]{\shortstack{$\mbox{Im} W_{-}$}}%
\special{ps: currentpoint grestore moveto}%
}
\put(3437,200){\makebox(0,0){0.7}}
\put(3034,200){\makebox(0,0){0.6}}
\put(2630,200){\makebox(0,0){0.5}}
\put(2227,200){\makebox(0,0){0.4}}
\put(1823,200){\makebox(0,0){0.3}}
\put(1420,200){\makebox(0,0){0.2}}
\put(1016,200){\makebox(0,0){0.1}}
\put(613,200){\makebox(0,0){0}}
\put(563,1913){\makebox(0,0)[r]{0.005}}
\put(563,1620){\makebox(0,0)[r]{0.003}}
\put(563,1327){\makebox(0,0)[r]{0.001}}
\put(563,1033){\makebox(0,0)[r]{-0.001}}
\put(563,740){\makebox(0,0)[r]{-0.003}}
\put(563,447){\makebox(0,0)[r]{-0.005}}
\end{picture}


==> fig2.tex <==
% GNUPLOT: LaTeX picture with Postscript
\setlength{\unitlength}{0.1bp}
\special{!
%!PS-Adobe-2.0 EPSF-2.0
%%Title: 're_v-av.tex'
%%Creator: gnuplot
%%DocumentFonts: 
%%BoundingBox: 0 0 288 216
%%Orientation: Landscape
%%EndComments
/gnudict 120 dict def
gnudict begin
/Color false def
/Solid false def
/gnulinewidth 5.000 def
/vshift -33 def
/dl {10 mul} def
/hpt 31.5 def
/vpt 31.5 def
/M {moveto} bind def
/L {lineto} bind def
/R {rmoveto} bind def
/V {rlineto} bind def
/vpt2 vpt 2 mul def
/hpt2 hpt 2 mul def
/Lshow { currentpoint stroke M
  0 vshift R show } def
/Rshow { currentpoint stroke M
  dup stringwidth pop neg vshift R show } def
/Cshow { currentpoint stroke M
  dup stringwidth pop -2 div vshift R show } def
/DL { Color {setrgbcolor Solid {pop []} if 0 setdash }
 {pop pop pop Solid {pop []} if 0 setdash} ifelse } def
/BL { stroke gnulinewidth 2 mul setlinewidth } def
/AL { stroke gnulinewidth 2 div setlinewidth } def
/PL { stroke gnulinewidth setlinewidth } def
/LTb { BL [] 0 0 0 DL } def
/LTa { AL [1 dl 2 dl] 0 setdash 0 0 0 setrgbcolor } def
/LT0 { PL [] 0 1 0 DL } def
/LT1 { PL [4 dl 2 dl] 0 0 1 DL } def
/LT2 { PL [2 dl 3 dl] 1 0 0 DL } def
/LT3 { PL [1 dl 1.5 dl] 1 0 1 DL } def
/LT4 { PL [5 dl 2 dl 1 dl 2 dl] 0 1 1 DL } def
/LT5 { PL [4 dl 3 dl 1 dl 3 dl] 1 1 0 DL } def
/LT6 { PL [2 dl 2 dl 2 dl 4 dl] 0 0 0 DL } def
/LT7 { PL [2 dl 2 dl 2 dl 2 dl 2 dl 4 dl] 1 0.3 0 DL } def
/LT8 { PL [2 dl 2 dl 2 dl 2 dl 2 dl 2 dl 2 dl 4 dl] 0.5 0.5 0.5 DL } def
/Pnt { stroke [] 0 setdash
   gsave 1 setlinecap M 0 0 V stroke grestore } def
/Dia { stroke [] 0 setdash 2 copy vpt add M
  hpt neg vpt neg V hpt vpt neg V
  hpt vpt V hpt neg vpt V closepath stroke
  Pnt } def
/Pls { stroke [] 0 setdash vpt sub M 0 vpt2 V
  currentpoint stroke M
  hpt neg vpt neg R hpt2 0 V stroke
  } def
/Box { stroke [] 0 setdash 2 copy exch hpt sub exch vpt add M
  0 vpt2 neg V hpt2 0 V 0 vpt2 V
  hpt2 neg 0 V closepath stroke
  Pnt } def
/Crs { stroke [] 0 setdash exch hpt sub exch vpt add M
  hpt2 vpt2 neg V currentpoint stroke M
  hpt2 neg 0 R hpt2 vpt2 V stroke } def
/TriU { stroke [] 0 setdash 2 copy vpt 1.12 mul add M
  hpt neg vpt -1.62 mul V
  hpt 2 mul 0 V
  hpt neg vpt 1.62 mul V closepath stroke
  Pnt  } def
/Star { 2 copy Pls Crs } def
/BoxF { stroke [] 0 setdash exch hpt sub exch vpt add M
  0 vpt2 neg V  hpt2 0 V  0 vpt2 V
  hpt2 neg 0 V  closepath fill } def
/TriUF { stroke [] 0 setdash vpt 1.12 mul add M
  hpt neg vpt -1.62 mul V
  hpt 2 mul 0 V
  hpt neg vpt 1.62 mul V closepath fill } def
/TriD { stroke [] 0 setdash 2 copy vpt 1.12 mul sub M
  hpt neg vpt 1.62 mul V
  hpt 2 mul 0 V
  hpt neg vpt -1.62 mul V closepath stroke
  Pnt  } def
/TriDF { stroke [] 0 setdash vpt 1.12 mul sub M
  hpt neg vpt 1.62 mul V
  hpt 2 mul 0 V
  hpt neg vpt -1.62 mul V closepath fill} def
/DiaF { stroke [] 0 setdash vpt add M
  hpt neg vpt neg V hpt vpt neg V
  hpt vpt V hpt neg vpt V closepath fill } def
/Pent { stroke [] 0 setdash 2 copy gsave
  translate 0 hpt M 4 {72 rotate 0 hpt L} repeat
  closepath stroke grestore Pnt } def
/PentF { stroke [] 0 setdash gsave
  translate 0 hpt M 4 {72 rotate 0 hpt L} repeat
  closepath fill grestore } def
/Circle { stroke [] 0 setdash 2 copy
  hpt 0 360 arc stroke Pnt } def
/CircleF { stroke [] 0 setdash hpt 0 360 arc fill } def
/C0 { BL [] 0 setdash 2 copy moveto vpt 90 450  arc } bind def
/C1 { BL [] 0 setdash 2 copy        moveto
       2 copy  vpt 0 90 arc closepath fill
               vpt 0 360 arc closepath } bind def
/C2 { BL [] 0 setdash 2 copy moveto
       2 copy  vpt 90 180 arc closepath fill
               vpt 0 360 arc closepath } bind def
/C3 { BL [] 0 setdash 2 copy moveto
       2 copy  vpt 0 180 arc closepath fill
               vpt 0 360 arc closepath } bind def
/C4 { BL [] 0 setdash 2 copy moveto
       2 copy  vpt 180 270 arc closepath fill
               vpt 0 360 arc closepath } bind def
/C5 { BL [] 0 setdash 2 copy moveto
       2 copy  vpt 0 90 arc
       2 copy moveto
       2 copy  vpt 180 270 arc closepath fill
               vpt 0 360 arc } bind def
/C6 { BL [] 0 setdash 2 copy moveto
      2 copy  vpt 90 270 arc closepath fill
              vpt 0 360 arc closepath } bind def
/C7 { BL [] 0 setdash 2 copy moveto
      2 copy  vpt 0 270 arc closepath fill
              vpt 0 360 arc closepath } bind def
/C8 { BL [] 0 setdash 2 copy moveto
      2 copy vpt 270 360 arc closepath fill
              vpt 0 360 arc closepath } bind def
/C9 { BL [] 0 setdash 2 copy moveto
      2 copy  vpt 270 450 arc closepath fill
              vpt 0 360 arc closepath } bind def
/C10 { BL [] 0 setdash 2 copy 2 copy moveto vpt 270 360 arc closepath fill
       2 copy moveto
       2 copy vpt 90 180 arc closepath fill
               vpt 0 360 arc closepath } bind def
/C11 { BL [] 0 setdash 2 copy moveto
       2 copy  vpt 0 180 arc closepath fill
       2 copy moveto
       2 copy  vpt 270 360 arc closepath fill
               vpt 0 360 arc closepath } bind def
/C12 { BL [] 0 setdash 2 copy moveto
       2 copy  vpt 180 360 arc closepath fill
               vpt 0 360 arc closepath } bind def
/C13 { BL [] 0 setdash  2 copy moveto
       2 copy  vpt 0 90 arc closepath fill
       2 copy moveto
       2 copy  vpt 180 360 arc closepath fill
               vpt 0 360 arc closepath } bind def
/C14 { BL [] 0 setdash 2 copy moveto
       2 copy  vpt 90 360 arc closepath fill
               vpt 0 360 arc } bind def
/C15 { BL [] 0 setdash 2 copy vpt 0 360 arc closepath fill
               vpt 0 360 arc closepath } bind def
/Rec   { newpath 4 2 roll moveto 1 index 0 rlineto 0 exch rlineto
       neg 0 rlineto closepath } bind def
/Square { dup Rec } bind def
/Bsquare { vpt sub exch vpt sub exch vpt2 Square } bind def
/S0 { BL [] 0 setdash 2 copy moveto 0 vpt rlineto BL Bsquare } bind def
/S1 { BL [] 0 setdash 2 copy vpt Square fill Bsquare } bind def
/S2 { BL [] 0 setdash 2 copy exch vpt sub exch vpt Square fill Bsquare } bind def
/S3 { BL [] 0 setdash 2 copy exch vpt sub exch vpt2 vpt Rec fill Bsquare } bind def
/S4 { BL [] 0 setdash 2 copy exch vpt sub exch vpt sub vpt Square fill Bsquare } bind def
/S5 { BL [] 0 setdash 2 copy 2 copy vpt Square fill
       exch vpt sub exch vpt sub vpt Square fill Bsquare } bind def
/S6 { BL [] 0 setdash 2 copy exch vpt sub exch vpt sub vpt vpt2 Rec fill Bsquare } bind def
/S7 { BL [] 0 setdash 2 copy exch vpt sub exch vpt sub vpt vpt2 Rec fill
       2 copy vpt Square fill
       Bsquare } bind def
/S8 { BL [] 0 setdash 2 copy vpt sub vpt Square fill Bsquare } bind def
/S9 { BL [] 0 setdash 2 copy vpt sub vpt vpt2 Rec fill Bsquare } bind def
/S10 { BL [] 0 setdash 2 copy vpt sub vpt Square fill 2 copy exch vpt sub exch vpt Square fill
       Bsquare } bind def
/S11 { BL [] 0 setdash 2 copy vpt sub vpt Square fill 2 copy exch vpt sub exch vpt2 vpt Rec fill
       Bsquare } bind def
/S12 { BL [] 0 setdash 2 copy exch vpt sub exch vpt sub vpt2 vpt Rec fill Bsquare } bind def
/S13 { BL [] 0 setdash 2 copy exch vpt sub exch vpt sub vpt2 vpt Rec fill
       2 copy vpt Square fill Bsquare } bind def
/S14 { BL [] 0 setdash 2 copy exch vpt sub exch vpt sub vpt2 vpt Rec fill
       2 copy exch vpt sub exch vpt Square fill Bsquare } bind def
/S15 { BL [] 0 setdash 2 copy Bsquare fill Bsquare } bind def
/D0 { gsave translate 45 rotate 0 0 Box stroke grestore } bind def
/D1 { gsave translate 45 rotate 0 0 S1 stroke grestore } bind def
/D2 { gsave translate 45 rotate 0 0 S2 stroke grestore } bind def
/D3 { gsave translate 45 rotate 0 0 S3 stroke grestore } bind def
/D4 { gsave translate 45 rotate 0 0 S4 stroke grestore } bind def
/D5 { gsave translate 45 rotate 0 0 S5 stroke grestore } bind def
/D6 { gsave translate 45 rotate 0 0 S6 stroke grestore } bind def
/D7 { gsave translate 45 rotate 0 0 S7 stroke grestore } bind def
/D8 { gsave translate 45 rotate 0 0 S8 stroke grestore } bind def
/D9 { gsave translate 45 rotate 0 0 S9 stroke grestore } bind def
/D10 { gsave translate 45 rotate 0 0 S10 stroke grestore } bind def
/D11 { gsave translate 45 rotate 0 0 S11 stroke grestore } bind def
/D12 { gsave translate 45 rotate 0 0 S12 stroke grestore } bind def
/D13 { gsave translate 45 rotate 0 0 S13 stroke grestore } bind def
/D14 { gsave translate 45 rotate 0 0 S14 stroke grestore } bind def
/D15 { gsave translate 45 rotate 0 0 S15 stroke grestore } bind def
/BoxFill { gsave Rec 1 setgray fill grestore } def
end
%%EndProlog
}
\begin{picture}(2880,2160)(0,0)
\special{"
gnudict begin
gsave
0 0 translate
0.100 0.100 scale
0 setgray
newpath
LTb
463 300 M
63 0 V
2191 0 R
-63 0 V
463 593 M
63 0 V
2191 0 R
-63 0 V
463 887 M
63 0 V
2191 0 R
-63 0 V
463 1180 M
63 0 V
2191 0 R
-63 0 V
463 1473 M
63 0 V
2191 0 R
-63 0 V
463 1767 M
63 0 V
2191 0 R
-63 0 V
463 2060 M
63 0 V
2191 0 R
-63 0 V
463 300 M
0 63 V
0 1697 R
0 -63 V
1027 300 M
0 63 V
0 1697 R
0 -63 V
1590 300 M
0 63 V
0 1697 R
0 -63 V
2154 300 M
0 63 V
0 1697 R
0 -63 V
2717 300 M
0 63 V
0 1697 R
0 -63 V
463 300 M
2254 0 V
0 1760 V
-2254 0 V
463 300 L
LT5
2341 623 Circle
1872 779 Circle
1590 902 Circle
1402 1005 Circle
1268 1096 Circle
1167 1174 Circle
1089 1244 Circle
LT6
2341 404 CircleF
1872 548 CircleF
1590 664 CircleF
1402 762 CircleF
1268 849 CircleF
1167 925 CircleF
1089 993 CircleF
LT2
638 2060 M
7 -26 V
23 -78 V
23 -70 V
22 -62 V
23 -57 V
23 -52 V
23 -48 V
23 -44 V
22 -41 V
23 -39 V
23 -36 V
23 -34 V
22 -32 V
23 -31 V
23 -29 V
23 -27 V
22 -26 V
23 -25 V
23 -24 V
23 -23 V
22 -22 V
23 -21 V
23 -21 V
23 -19 V
23 -19 V
22 -18 V
23 -18 V
23 -17 V
23 -17 V
22 -16 V
23 -15 V
23 -15 V
23 -15 V
22 -14 V
23 -14 V
23 -13 V
23 -13 V
23 -13 V
22 -13 V
23 -12 V
23 -12 V
23 -11 V
22 -12 V
23 -11 V
23 -10 V
23 -11 V
22 -10 V
23 -11 V
23 -10 V
23 -9 V
23 -10 V
22 -9 V
23 -10 V
23 -9 V
23 -9 V
22 -8 V
23 -9 V
23 -8 V
23 -9 V
22 -8 V
23 -8 V
23 -8 V
23 -8 V
23 -7 V
22 -8 V
23 -7 V
23 -8 V
23 -7 V
22 -7 V
23 -7 V
23 -7 V
23 -7 V
22 -7 V
23 -7 V
23 -6 V
23 -7 V
22 -6 V
23 -7 V
23 -6 V
23 -6 V
23 -6 V
22 -7 V
23 -6 V
23 -6 V
23 -6 V
22 -6 V
23 -5 V
23 -6 V
23 -6 V
22 -6 V
23 -5 V
23 -6 V
LT3
584 2060 M
16 -85 V
22 -105 V
23 -90 V
23 -79 V
23 -70 V
22 -63 V
23 -57 V
23 -52 V
23 -48 V
23 -44 V
22 -41 V
23 -39 V
23 -35 V
23 -34 V
22 -32 V
23 -30 V
23 -29 V
23 -27 V
22 -25 V
23 -25 V
23 -23 V
23 -23 V
22 -21 V
23 -21 V
23 -20 V
23 -19 V
23 -18 V
22 -18 V
23 -17 V
23 -16 V
23 -16 V
22 -15 V
23 -15 V
23 -15 V
23 -14 V
22 -13 V
23 -14 V
23 -12 V
23 -13 V
23 -12 V
22 -12 V
23 -11 V
23 -12 V
23 -10 V
22 -11 V
23 -11 V
23 -10 V
23 -10 V
22 -10 V
23 -9 V
23 -9 V
23 -10 V
23 -9 V
22 -8 V
23 -9 V
23 -8 V
23 -9 V
22 -8 V
23 -8 V
23 -8 V
23 -7 V
22 -8 V
23 -7 V
23 -8 V
23 -7 V
23 -7 V
22 -7 V
23 -7 V
23 -7 V
23 -7 V
22 -6 V
23 -7 V
23 -6 V
23 -7 V
22 -6 V
23 -6 V
23 -6 V
23 -6 V
22 -6 V
23 -6 V
23 -6 V
23 -6 V
23 -6 V
22 -5 V
23 -6 V
23 -5 V
23 -6 V
22 -5 V
23 -6 V
23 -5 V
23 -6 V
22 -5 V
23 -5 V
23 -5 V
stroke
grestore
end
showpage
}
\put(1590,50){\makebox(0,0){$r=a_f/a$}}
\put(100,1180){%
\special{ps: gsave currentpoint currentpoint translate
270 rotate neg exch neg exch translate}%
\makebox(0,0)[b]{\shortstack{$Re W_{-}^{\Sigma}$}}%
\special{ps: currentpoint grestore moveto}%
}
\put(2717,200){\makebox(0,0){0.4}}
\put(2154,200){\makebox(0,0){0.3}}
\put(1590,200){\makebox(0,0){0.2}}
\put(1027,200){\makebox(0,0){0.1}}
\put(463,200){\makebox(0,0){0}}
\put(413,2060){\makebox(0,0)[r]{6}}
\put(413,1767){\makebox(0,0)[r]{5.5}}
\put(413,1473){\makebox(0,0)[r]{5}}
\put(413,1180){\makebox(0,0)[r]{4.5}}
\put(413,887){\makebox(0,0)[r]{4}}
\put(413,593){\makebox(0,0)[r]{3.5}}
\put(413,300){\makebox(0,0)[r]{3}}
\end{picture}

